Building a Cultural Perspective on Doctor-Patient Conversations

AI-powered medical scribes are increasingly used to transcribe doctor-patient conversations and automate clinical documentation. However, large-scale real-world consultation datasets are scarce due to the sensitivity of clinical conversations, leading developers to rely on simulated and LLM-generated synthetic consultations. While scalable, these alternatives may fail to capture culturally situated patterns of clinical interaction. We introduce interactional cultural markers, measurable patterns of doctor-patient interaction grounded in cross-cultural clinical communication, and use them to compare real, simulated, and synthetic consultations from Indian and US clinical contexts. We find distinct patterns of participation and control: Indian consultations involve greater patient participation but stronger doctor control, while US consultations exhibit balanced participation and open-ended discussion. Synthetic Indian consultations often fail to reproduce these patterns, instead converging toward US-like interaction. We identify additional synthetic signatures, including excessive doctor explanation and formulaic patient responses. We conclude by discussing implications for generating culturally grounded synthetic clinical conversations.

==> Sections/old-discussion.tex <==
\section{Discussion}

Our results establish: clinical consultations differ systematically in interactional structure across cultural settings, and synthetic clinical consultations reproduces some of these differences while flattening or misrepresenting others. These different settings allow us to examine broader differences in how control, participation, and interaction are organized across consultations. These findings also provide perspectives for designing and evaluating clinical dialogue data that more faithfully captures the interactional practices of the settings it is intended to represent.

% Just trying to walk through my understanding. I am first trying to establish that the markers we observed are representative of culture. With this, I am trying use this as a baseline to say how synthetic data is not modelled well, and why that might be the case, and finally I'm talking about how to model such data well, inspired from our markers. 

\subsection{Understanding Interactional Culture in Clinical Interaction}

The comparison between Indian and US consultations suggests that the key distinction lies in how interactional control and participation are distributed in clinical conversations. Higher doctor directiveness and interruption rates in Indian consultations highlight a pattern in which doctors guide the progression of an extended patient narrative. In contrast, US consultations show a more balanced distribution, with doctors contributing more conversational material while giving patients greater scope to narrate through open-ended questioning. This difference may reflect the practical conditions of Indian outpatient care, where high patient volumes result in constrained consultation times \cite{mehradoctorinfluence}, making directive questioning and quick redirection practical mechanisms for maintaining clinical efficiency. In contrast, US clinical communication more strongly emphasizes beginning consultations with broad questions that allow patients to present their concerns in their own terms \cite{westernconsultationMarvel}; a large-sample analyses similarly characterize US doctor-patient communication as negotiated, patient-centered exchange rather than tightly bounded question sequences \cite{roterstewart1997}, consistent with the stronger patient-initiated questioning and negotiation observed in our US consultations.

The observed Indian patterns in our markers also strongly correspond to properties described in the literature. The higher directiveness scores, built on short, bounded doctor questions, align with prior audits reporting that Indian doctor-patient interactions lean heavily on closed rather than discursive questioning \cite{doctorbehaviour}. The lower rate of formal \textit{Symptom Description} among Indian patients, and the visible colloquial framing, relate to studies patients describing illness through everyday idiom rather than clinical terminology \cite{idiomsofdistress}. The code-mixing patterns with clinical concepts introduced through switches between English and the regional language, match prior descriptions \cite{codemixing}. These qualitative observations recurring as measurable, cross-dataset, and cross-culture regularities in our framework is suggestive evidence that the markers are picking up real interactional structure rather than dataset-specific artifacts.

\subsection{Synthetic Signatures: The Limits of Generated Realism}

Across languages and cultural prompts, synthetic consultations tend to move toward a common interactional configuration that is distinct from the real and simulated consultations. Synthetic generation frameworks built on LLMs, which are optimized for fluent written text, have been shown to struggle to reproduce the natural rhythm, emotional expressiveness, and turn-taking dynamics of genuine spoken interaction \cite{mayorllmconversations2025, haider2025synthetic}. These findings complement our flagged verbosity, elaborated question, and high certainty patient responses to suggest that synthetic clinical dialogue can appear highly coherent but imposes its own conversational regularities on the clinical encounter.

The synthetic Indian dialogues reveal a further distinction in how culture is interpreted in the Indian context. The repeated, sometimes gender- or age-inappropriate use of kinship terms as address by synthetic doctors may reflect the broader conversational use of kinship terms as conversational address in Indian languages \cite{indianenglish2019}. This could potentially be carried into clinical dialogue by the model even when the specific address is contextually inappropriate. Similarly, the pattern of over-compliance and gratitude may reflect documentation of doctor--patient relationships historically that have linked patients' deference, respect, and trust toward physicians to the elevated social status and authority associated with the medical profession \cite{kumbhar2024doctors}. The recurrence of these cues in synthetic dialogue may indicate that such associations can be carried into contemporary everyday clinical language, where they surface as heightened gratitude, deference, reassurance, and culturally marked forms of address.

\subsection{Design Implications for Culturally Grounded Clinical Data}

Beyond documenting these gaps, the framework identifies explicit weaknesses in clinical data and points generation pipelines toward targeted fixes, such as improved grounding or realism constraints. Ensuring synthetic data is culturally representative is also particularly important because inaccurately modeled interactional characteristics can propagate into downstream clinical systems, where errors in speech interpretation and documentation may affect the clinical record and patient care \cite{Gonzalez_Iniguez_Jung_Lee_Bell_Arroyo_2026}.

\subsubsection{Modeling synthetic clinical dialogue}

The observed synthetic signatures suggest several interactional dimensions that can be explicitly modeled when generating clinical dialogue. Generation pipelines should separate clinical from interactional grounding: clinical notes can specify symptoms, history, and medical facts, while interactional constraints guide how these are elicited and expressed. Generation should also guard against unsupported synthetic signatures, including systematic over-explanation, unprompted reassurance, excessive empathy, unusually confident patient responses, and culturally marked expressions. The aim is not to remove legitimate empathy, gratitude, or culturally specific address, but to prevent them from becoming default proxies for cultural authenticity.

\subsubsection{Generating Indian clinical dialogue} For culturally grounded Indian doctor--patient conversations, cultural grounding must operate at the level of interaction, not only vocabulary. Datasets should preserve how doctors question, redirect, and interrupt; how patients elaborate beyond questions; and how clinical information is expressed through everyday language and code-switching. This argues against constructing an ``Indian'' dataset primarily by translating Western consultations or adding Indian names, languages, and culturally recognizable expressions~\cite{indicmeddialog2026}, which can reproduce surface cues while retaining the source setting's interactional structure.

For simulated data, role-play instructions should therefore specify interactional expectations alongside clinical content: patients should be able to provide trailing or unsolicited information, doctors should redirect or constrain narratives where appropriate, and histories should emerge through colloquial or code-mixed descriptions. The goal is to make the conversation a little more chaotic and real, and these markers should define distributions rather than rigid rules, given the heterogeneity of Indian clinical settings.

\subsubsection{Evaluating existing synthetic data} The framework also enables evaluation after dataset construction. Rather than assigning a single overall ``realism'' score, developers can compare distributions of interactional cultural markers against appropriate real or simulated reference data to identify fine-grained deviations. Prompts, generation strategies, sampling procedures, or filtering rules can then be revised for markers showing large differences, followed by re-evaluation to assess whether cultural fidelity improved without introducing new synthetic signatures. This shifts cultural evaluation from subjective post-hoc judgment toward iterative quality control.


The broader implication is therefore that clinical dialogue data should be evaluated on two dimensions: whether the conversation is clinically plausible, and whether it is interactionally faithful to the setting in which it is intended to be used. For newly collected or generated data, this requires preserving culturally situated interaction during collection and annotation; for synthetic data, combining clinical grounding with interactional validation and artefact controls; and for existing datasets, auditing marker distributions against appropriate real or simulated references This motivates cultural fidelity as a measurable, phase-aware modeling objective, guiding models toward culturally grounded participation, interaction, and responsiveness while reducing generic clinical schemas and exaggerated cultural associations.



==> Sections/rough.tex <==
Methodology

%We use patterns from this literature to build our cultural markers: transcript-level properties that can be measured and compared across conversations. This follows prior work of coding medical dialogue into observable interactional behaviors, exemplified by instruments such as the Roter Interaction Analysis System \cite{riasroter}. The markers are not intended to constitute a definition of Indian communication, nor does the presence or absence of any individual marker provide a binary test of cultural identity. Rather, they provide reference points for examining how strongly these interactional characteristics are expressed in doctor-patient conversations in a particular cultural setting, and how their prevalence varies across cultures. They also allow us to examine the extent to which synthetic conversations reproduce, exaggerate, or omit these characteristics.


% Literature
% Doctor–patient communication has long been studied using structured coding frameworks that decompose consultations into observable interactional behaviors. The Roter Interaction Analysis System (RIAS), for example, categorizes physician and patient utterances across task-oriented and socioemotional dimensions \cite{riasroter}. The Four Habits Coding Scheme instead focuses on clinician communication through four broad components: investing in the beginning, eliciting the patient’s perspective, demonstrating empathy, and investing in the end \cite{krupat2006four}. A systematic review of physician–patient communication measures identifies a range of established frameworks, including RIAS, the Byrne and Long classification, the Four Habits Coding Scheme, SEGUE, and other communication coding systems \cite{zill2014measurement}. 

% Beyond healthcare, research on culturally aware dialogue similarly shows that culture is expressed through multiple interacting dimensions of conversational behavior.. The Culturally-Aware Conversations framework uses established cultural dimensions like power distance to predict which stylistic axis — directness, self-disclosure, deference — should vary most across cultures for a given situation~\cite{havaldar2025culturally}. A broader Cultural Context Schema for grounding social norms and their violations has similarly been proposed and validated against everyday conversation~\cite{pujari2025llmhuman}, and earlier work represented culture via Hofstede survey dimensions fused into dialogue-agent encodings~\cite{cao2024bridging}. However, clinical dialogue is shaped by its own roles, expertise asymmetries, and medical goals which are different from everyday conversation \cite{tenhave1991talk, pilnick2011remarkable}, motivating dedicated grounding, definitions and examination of cultural variation.

% intro

% These systems rest on an important assumption: that the data used to train and/or validate their underlying models adequately represents the clinical interactions they will encounter in practice. However, LLMs have been shown to exhibit data-centric biases when applied across culturally distinct contexts~\cite{naous-etal-2024-beer,adilazuarda-etal-2024-towards}. In practice, such differences can affect whether a system correctly interprets colloquial symptom descriptions, handles code-switching within an utterance, or produces clinical documentation that faithfully reflects the interaction~\cite{codemixing}.

%Yet the validity of synthetic data as a substitute for real clinical interaction in a cultural context has not been examined. Existing evaluations consider overall realism, medical accuracy, and persona consistency~\cite{haider2025synthetic}, but do not establish whether generated consultations fairly represent participation and linguistic behavior in a particular cultural setting--dimensions that prior work has shown to vary significantly between different clinical contexts~\cite{roter2003communication, doctorbehaviour, mehradoctorinfluence}. If these interactional properties are not reproduced, synthetic data used to train or evaluate clinical AI systems may produce biased output in downstream tasks.
% or amplify the mismatches for the settings they are intended to model. 

% To address this, we propose a layered framework for evaluating cultural realism in the clinical context of doctor-patient conversation, defined as the extent to which clinical dialogue reflects interactional patterns observed in a given cultural context, operationalizing it through multiple observable dimensions of interaction. We apply it across real, simulated, and LLM-generated synthetic consultations in English, Hindi, and Telugu. Figure~\ref{fig:example_consultation} illustrates an example of these dimensions, highlighting interactional patterns that distinguish real Western and Indian consultations from LLM-generated dialogue.

% % 
% Our key contributions are as follows:
% \begin{itemize}
%     \item \textbf{A multi-level framework for interactional comparison}. We develop a framework that captures multiple dimensions of doctor–patient interaction, including conversational participation and control, directiveness, patient information sharing, response behavior, interruptions, and linguistic register.
    
%     \item \textbf{An empirical characterization of Indian–Western variation:} We systematically compare clinical conversations from Indian and Western settings to identify interactional properties that distinguish the two contexts, 
%     quantifying where and how they diverge.
    
%     \item \textbf{An evaluation of cultural reproduction in synthetic dialogue.} We evaluate synthetic clinical conversations across languages and generation settings, measuring which interactional properties are reproduced, weakened, or introduced by synthetic generation and identifying systematic departures from observed clinical interactions.
% \end{itemize}

%Beyond healthcare, culturally aware dialogue research treats culture as multidimensional: Culturally-Aware Conversations uses dimensions such as power distance to predict variation in directness, self-disclosure, and deference \cite{havaldar2025culturally}, while the Cultural Context Schema grounds social norms and their violations in everyday conversation, and earlier work incorporates Hofstede dimensions into dialogue-agent representations \cite{pujari2025llmhuman,cao2024bridging}. However, clinical dialogue is shaped by domain-specific roles, expertise asymmetries, and medical goals that distinguish it from everyday conversation \cite{tenhave1991talk,pilnick2011remarkable}, motivating dedicated approaches to grounding and examining cultural variation in clinical interaction.

%We use learning from prior work to define our proposed \textbf{cultural markers}: measurable properties of doctor-patient conversations that capture interactional behaviour. This follows established approaches to coding medical interaction, including the Roter Interaction Analysis System (RIAS) and the Four Habits Coding Scheme \cite{riasroter,krupat2006four}. These are general-purpose frameworks designed for coding doctor-patient communication universally. Rather than treating any individual marker as representative of a cultural group, we use these measures as reference points for comparing Indian and Western consultations and for examining whether synthetic conversations reproduce, exaggerate, or omit interactional patterns observed in real and simulated clinical data.

% \subsection{Cultural Markers}

\section{Metric Definitions}
\label{app:metrics}

We provide complete definitions for all metrics used in the framework,
organised by layer. For each metric we specify the unit of measurement,
what constitutes a positive instance, and the label set or scale used
during annotation. All metrics were first defined operationally,
piloted on a held-out set of five conversations per language, and then
revised through two rounds of feedback from clinical experts --- one
practising physician and one clinical communication researcher --- before
being applied to the full corpus.

\subsection{L0 --- Surface-Level Distributional Metrics}
\label{app:metrics:l0}

These metrics are computed directly from the transcript without
model-based annotation, using token counts and a curated word list.

\medskip
\noindent\textbf{Doctor-to-Patient Word Ratio (D:P ratio).}
Computed as the total word count of all doctor turns divided by the
total word count of all patient turns across the conversation. Values
below 1.0 indicate patient-dominant speech; values above 1.0 indicate
doctor-dominant speech. Words are counted after stripping punctuation
and normalising whitespace; for Hindi and Telugu, whitespace-delimited
tokens serve as the counting unit.

\medskip
\noindent\textbf{History-Taking to Treatment Turn Ratio (HT:Tx ratio).}
Computed as the number of turns assigned to the History Taking phase
divided by the number of turns assigned to the Treatment\,/\,Prescription
phase (from the phase segmentation). Higher ratios reflect
consultations in which more of the conversational work is devoted to
elicitation before moving to clinical action. Prior studies of Indian
outpatient care report that consultations are brief and heavily
weighted toward rapid history elicitation~\cite{waitingtimedas},
which this ratio operationalizes.

\medskip
\noindent\textbf{Turn-Length Uniformity.}
Measured as the coefficient of variation (standard deviation divided by
mean) of word counts across all turns, computed separately for doctor
and patient turns. Low variance flags artificially regular synthetic
pacing; high variance is characteristic of real consultations, where
brief acknowledgments sit alongside extended narrations.

\medskip
\noindent\textbf{Backchannel Rate.}
The proportion of turns --- across both speakers --- whose entire
content consists of a backchannel or minimal acknowledgment token. The
token list covers: \textit{okay, yes, sure, right, hmm, mm-hmm, fine,
of course, I see, understood}, and their transliterated equivalents in
Hindi and Telugu (e.g., \textit{achha, theek hai, arey, sare}). A turn
qualifies if, after stripping punctuation, its normalised content
matches an item in this list.

\medskip
\noindent\textbf{Vocative Frequency (Patient).}
The proportion of patient turns containing a direct address term for
the doctor. The term list includes \textit{sir, doctor, doctor sahab,
sahab} and script-native equivalents: Hindi
{\devanagarifont सर, डॉक्टर साहब}; Telugu {\telugufont సర్, డాక్టర్ సాహబ్,
అయ్యా}. Annotated as a count per turn; reported as a proportion
across all patient turns in the conversation. The use of honorific
address in Indian clinical encounters reflects the elevated social
status and authority historically associated with the medical
profession in India~\cite{kumbhar2024doctors}, and provides a
measurable signal for the asymmetric power dynamic documented in
Indian doctor--patient interaction~\cite{powerimabalance2006}.

\subsection{Phase Identification}
\label{app:metrics:phase}

Each turn is assigned to exactly one consultation phase prior to
applying the multi-level analysis, following the Byrne and Long
framework~\cite{byrne1976doctors} extended as described in
Section~\ref{sec:methodology}. Phase labels provide contextual
grounding for the interactional measures --- for example, doctor
terseness during history taking indicates directive questioning, while
the same terseness during treatment indicates efficient prescription
rather than interrogation. Table~\ref{tab:phase-codes} lists the codes
and their operational definitions.

\begin{table}[h]
\small
\caption{Consultation phase codes and operational definitions.}
\label{tab:phase-codes}
\begin{tabular}{@{}lll@{}}
\toprule
\textbf{Code} & \textbf{Phase} & \textbf{Operational definition} \\
\midrule
GR & Greeting
  & Initial pleasantries; no clinical content \\
SE & Social Exchange
  & Non-clinical chit-chat before clinical content begins \\
CC & Chief Complaint
  & First turn(s) in which the patient states the primary reason \\
HT & History Taking
  & Elicitation of onset, duration, severity, associated symptoms, \\
  &
  & past medical history, family or social history \\
PE & Physical Examination
  & Doctor initiates, conducts, or narrates an examination; \\
  &
  & patient responds to examination instructions \\
DX & Diagnosis\,/\,Explanation
  & Doctor explains findings, offers a differential, or announces \\
  &
  & a diagnosis \\
TX & Treatment\,/\,Prescription
  & Doctor prescribes medication, orders investigations, \\
  &
  & or advises lifestyle changes \\
CL & Closing\,/\,Follow-up
  & Wrap-up, follow-up scheduling, farewell \\
\bottomrule
\end{tabular}
\end{table}

\noindent Each turn was assigned phase labels. Where a single turn
spanned two phases (e.g., a closing remark appended to a prescription),
the all phases were recorded.

\subsection{L1 --- Inter-Turn Dynamics}
\label{app:metrics:l1}

These metrics examine how speakers respond to one another across turn
boundaries, characterizing how they coordinate their contributions and
manage the progression of the interaction.

\medskip
\noindent\textbf{Interruption Rate}
The proportion of turns that interrupt an ongoing or trailing turn per speaker. An interruption is coded when:In transcripts, interruptions may also be flagged
by overlapping speech markers or dashes in the source. Reported as a
proportion of all doctor turns. The directive style documented in
Indian clinical encounters~\cite{mehradoctorinfluence}, in which
doctors actively guide the interaction across consultation phases,
motivates this as a measurable signal of interactional control.

\medskip
\noindent\textbf{Doctor Echo.}
The proportion of doctor turns in which the doctor explicitly repeats
or closely reformulates a word or phrase from the immediately preceding
patient turn, functioning as a confirmation or redirection device.
E.g., Patient: \textit{``\ldots neck stiffness\ldots''} $\to$ Doctor:
\textit{``This neck stiffness --- were you doing something at the
time?''}

\medskip
\noindent\textbf{Topic Continuity.}
Annotated per adjacent turn pair. Coded as \textit{Continuous} if the
doctor's turn takes up the clinical topic introduced or extended by the
patient's preceding turn; \textit{Discontinuous} if the doctor's turn
shifts to a new topic without acknowledging the patient's contribution.
This captures whether doctors follow the patient's narrative thread or
redirect it, distinguishing the patient-centered open-ended structure
documented in US consultations~\cite{roterstewart1997} from the more
bounded exchanges observed in Indian outpatient care~\cite{doctorbehaviour}.

\medskip
\noindent\textbf{Question--Answer Uptake.}
Coded per question-answer pair. Uptake is present when the doctor's
immediately following turn explicitly acknowledges, builds on, or uses
the information provided in the patient's answer before moving to the
next question. Absence of uptake --- moving directly to the next
question without acknowledgment --- is coded as \textit{No uptake}.
Low uptake is consistent with the tightly bounded, closed questioning
style documented in Indian outpatient consultations~\cite{doctorbehaviour}.

\subsection{L2 --- Turn-Level Metrics}
\label{app:metrics:l2}

For each metric, a single turn is provided to the model for
annotation. A single turn consists of a doctor utterance and a patient
response. For repeated exchanges within a turn, annotation takes the
first doctor utterance to the last patient utterance after the first
speaker switch. Even for speaker-specific metrics, the interlocutor's
contribution is provided as context --- for example, annotating whether
a patient response is trailing requires knowing the type of question
the doctor asked.

\subsubsection*{2A.\; Tone (Doctor)}

Annotated per turn;Inspired by studies observing Indian doctor--patient
conversations to be short and directive~\cite{waitingtimedas,doctorbehaviour}
and US consultations to emphasize open-ended questioning and
collaborative framing~\cite{westernconsultationMarvel,roterstewart1997}.
The \emph{Directiveness} metric reported in Table~\ref{tab:dataset-characteristics}
is the proportion of all doctor turns labelled Directive (exclusive or
alongside other labels).

\begin{table}[h]
\small
\caption{Tone labels (doctor turns; multi-select).}
\label{tab:tone}
\begin{tabular}{@{}p{2.2cm}p{4.8cm}p{4.2cm}@{}}
\toprule
\textbf{Label} & \textbf{Definition} & \textbf{Example} \\
\midrule
Directive
  & Issues an instruction or command; no rationale offered
  & \textit{``Take this twice a day.''} \\[2pt]
Discussive
  & Explains reasoning, invites questions, or frames the exchange
    as collaborative
  & \textit{``I'm giving you this because it reduces inflammation ---
    any questions?''} \\[2pt]
Empathetic
  & Explicitly acknowledges, validates, or responds to the patient's
    emotional state or circumstances
  & \textit{``I understand this has been worrying for you.''} \\
\bottomrule
\end{tabular}
\end{table}
\subsubsection*{2B.\; Verbosity (Doctor)}

Annotated per turn on a three-point scale. Inspired by Indian studies
reporting that doctors ask short, directive questions with little
elaboration~\cite{doctorbehaviour}, in contrast to the over-explanatory
synthetic signatures we document. The \emph{Verbosity} metric is the
proportion of doctor turns labelled \textit{Overly verbose}.

\begin{table}[h]
\small
\caption{Verbosity scale (doctor turns).}
\label{tab:verbosity}
\begin{tabular}{@{}lp{4.0cm}p{3.8cm}@{}}
\toprule
\textbf{Label} & \textbf{Definition} & \textbf{Example} \\
\midrule
Terse
  & Short and direct; no elaboration beyond what the clinical purpose
    requires
  & \textit{``Any fever?''} \\[4pt]
Appropriate
  & Natural amount of context or rationale; not padded, not bare
  & \textit{``I'm asking about your diet because sodium can worsen
    blood pressure.''} \\[4pt]
Overly verbose
  & More elaboration, repetition, or framing than the clinical
    situation requires
  & \textit{``So what I'm going to do is, given everything you've
    described\ldots''} \\
\bottomrule
\end{tabular}
\end{table}

\subsubsection*{2C.\; Question Structure (Doctor)}

Annotated per doctor turn; turns containing no question are labelled
N/A. The combination of multiple unrelated questions within a single
turn is a recurring synthetic artefact we document, contrasting with
the single, bounded questions characteristic of real Indian
consultations~\cite{doctorbehaviour}. The \emph{Question Structure}
metric is the proportion of doctor turns labelled \textit{Multiple
unrelated questions}.

\begin{table}[h]
\small
\caption{Question structure labels (doctor turns).}
\label{tab:qstruct}
\begin{tabular}{@{}p{3.8cm}p{4.2cm}p{3.2cm}@{}}
\toprule
\textbf{Label} & \textbf{Definition} & \textbf{Example} \\
\midrule
Single question
  & One question in the turn
  & \textit{``Any fever?''} \\[4pt]
Multiple related questions
  & Several questions on the same symptom or topic
  & \textit{``Do you have fever? Any cough? Vomiting?''} \\[4pt]
Multiple unrelated questions
  & Several questions spanning distinct clinical topics
  & \textit{``How is your BP? Also, sleeping well?''} \\[4pt]
N/A & No question present & --- \\
\bottomrule
\end{tabular}
\end{table}

\subsubsection*{2D.\; Language\,/\,Register (Doctor and Patient)}

Grounded in prior descriptions of Indian patients describing illness
through everyday idiom and folk language rather than clinical
terminology~\cite{idiomsofdistress}, and of heavy code-mixing in
Indian clinical encounters~\cite{codemixing}. The \emph{Register}
metric for doctors is the proportion of doctor turns containing at
least one Formal clinical label.

\begin{table}[h]
\small
\caption{Register labels (doctor and patient turns; multi-select).}
\label{tab:register}
\begin{tabular}{@{}p{3.2cm}p{4.6cm}p{3.4cm}@{}}
\toprule
\textbf{Label} & \textbf{Definition} & \textbf{Example} \\
\midrule
Formal clinical
  & Formal medical vocabulary dominates
  & \textit{``bilateral pedal oedema''} \\[3pt]
Colloquial
  & Everyday, informal phrasing
  & \textit{``pain here,'' ``feeling off''} \\[3pt]
Regional\,/\,vernacular
  & Regional-language or folk terms for illness
  & \textit{``sugar disease,'' ``stomach fire''} \\[3pt]
Medical shorthand
  & Common clinical abbreviations; not formal, not regional
  & \textit{``BP,'' ``Hb,'' ``USG''} \\[3pt]
N/A & No clinical or register content to assess & --- \\
\bottomrule
\end{tabular}
\end{table}

\subsubsection*{2E.\; Patient Response Style}

Annotated per turn following a doctor question. Indian patients have
been observed to provide extended narratives beyond the immediate
question~\cite{mehradoctorinfluence}, which this marker captures as
the Trailing label. The \emph{Trailing Responses} metric is the
proportion of patient turns labelled Trailing.

\begin{table}[h]
\small
\caption{Response style labels (patient turns).}
\label{tab:response-style}
\begin{tabular}{@{}p{2.4cm}p{5.0cm}p{3.8cm}@{}}
\toprule
\textbf{Label} & \textbf{Definition} & \textbf{Example} \\
\midrule
Structured
  & Directly and completely answers the question; no drift
  & \textit{``It started two days ago.''} \\[4pt]
Trailing
  & Begins to answer but drifts, repeats, or extends into unsolicited
    narrative
  & \textit{``Yes, it started\ldots I mean it comes and goes, and at
    night it's worse, and I also have this other thing\ldots''} \\[4pt]
Deflecting
  & Avoids the question or pivots to a different topic
  & D: \textit{``Any fever?''} / P: \textit{``I've been very tired
    lately.''} \\
\bottomrule
\end{tabular}
\end{table}

\subsubsection*{2F.\; Information Volunteering (Patient)}

Annotated per patient turn following a doctor question. Captures
whether patients extend their responses beyond what is explicitly
requested, consistent with the extended patient narratives documented
in Indian consultations~\cite{mehradoctorinfluence} even under
directive questioning.

\begin{table}[h]
\small
\caption{Information volunteering labels (patient turns).}
\label{tab:info-vol}
\begin{tabular}{@{}p{2.2cm}p{5.2cm}p{3.8cm}@{}}
\toprule
\textbf{Label} & \textbf{Definition} & \textbf{Example} \\
\midrule
Exact
  & Answers only what was directly asked; nothing more
  & D: \textit{``Any fever?''} / P: \textit{``Yes.''} \\[4pt]
Add-on
  & Answers the question and spontaneously volunteers additional
    relevant information the doctor did not ask for
  & D: \textit{``Any fever?''} / P: \textit{``Yes, and I've also had
    a cough since yesterday.''} \\[4pt]
N/A & Not a question-answer turn & --- \\
\bottomrule
\end{tabular}
\end{table}

\subsubsection*{2G.\; Symptom Description (Patient)}

Annotated per patient turn in which a symptom is mentioned. Grounded
in prior accounts of Indian patients describing illness through
everyday idiom and metaphor rather than clinical
terminology~\cite{idiomsofdistress} --- for example, \textit{sir fata
ja raha hai} (``my head is splitting'') as a colloquial description of
headache. The contrast between colloquial and clinical framing is a
key marker distinguishing Indian from US patient speech in our corpus.

\begin{table}[h]
\small
\caption{Symptom description labels (patient turns).}
\label{tab:symptom-desc}
\begin{tabular}{@{}p{2.8cm}p{4.8cm}p{3.6cm}@{}}
\toprule
\textbf{Label} & \textbf{Definition} & \textbf{Example} \\
\midrule
Gesture\,/\,Deictic
  & Points or uses spatial or demonstrative language
  & \textit{``It hurts here.''} / \textit{``Like this, when I press
    it.''} \\[3pt]
Clinical
  & Uses a medical or technical term for the symptom
  & \textit{``I have palpitations.''} \\[3pt]
Colloquial
  & Uses everyday or folk language for the symptom
  & \textit{``My stomach is on fire.''} / \textit{``My head is
    splitting.''} \\[3pt]
N/A & No symptom description in this turn & --- \\
\bottomrule
\end{tabular}
\end{table}

\subsubsection*{2H.\; Patient Response to Recommendation}

Annotated on patient turns following a DX or TX doctor
turn as given in Table \ref{tab:rec-response}. The low rate of patient questioning and high agreement rate
observed in Indian consultations~\cite{powerimabalance2006} is
captured here through the Accepts label; the remaining labels capture
the richer negotiation and questioning documented in US
consultations~\cite{roterstewart1997}. The \emph{Response-Agreement}
metric is the proportion of patient DX/TX-response turns labelled
\textit{Accepts} only (i.e., without any other label co-occurring).

\begin{table}[h]
\small
\caption{Response to recommendation labels (patient turns; multi-select).}
\label{tab:rec-response}
\begin{tabular}{@{}p{3.4cm}p{4.8cm}p{3.0cm}@{}}
\toprule
\textbf{Label} & \textbf{Definition} & \textbf{Example} \\
\midrule
Accepts
  & Agrees without asking any clarifying question
  & \textit{``Okay, doctor.''} \\[3pt]
Accepts with clarification
  & Agrees but asks a practical follow-up
  & \textit{``How long will I need to take this?''} \\[3pt]
Questions
  & Asks about the recommendation without clear resistance or acceptance
  & \textit{``Preeclampsia? What does that mean?''} \\[3pt]
Expresses concern\,/\,fear
  & Hesitates out of worry about treatment or its effects
  & \textit{``Will this medicine harm the baby?''} \\[3pt]
Refuses
  & Explicitly declines the recommendation
  & \textit{``I don't want to take medication.''} \\[3pt]
Disagrees
  & Pushes back on the diagnosis or recommendation itself
  & \textit{``I don't think it's that serious.''} \\[3pt]
Misunderstands
  & Response indicates a mistaken understanding of what was said
  & D: \textit{``Once daily.''} / P: \textit{``I'll take it whenever
    I feel bad.''} \\[3pt]
Provides alternative information
  & Counters or supplements with information from another source
  & \textit{``My neighbour said this is normal.''} \\[3pt]
Unclear & Does not fit another category & --- \\[2pt]
N/A & Not a response to a DX/TX turn & --- \\
\bottomrule
\end{tabular}
\end{table}

\subsubsection*{2I.\; Patient Certainty}

Annotated per patient turn that constitutes a factual answer to a
history or symptom question. High certainty in synthetic patient
responses --- patients providing clean, confident answers rather than
the hedging and qualification that naturally occur in clinical
histories --- is a recurring synthetic signature we document across
languages. The \emph{Certainty} metric is the proportion of patient
history-answer turns labelled Certain.

\begin{table}[h]
\small
\caption{Certainty labels (patient turns).}
\label{tab:certainty}
\begin{tabular}{@{}p{3.0cm}p{5.0cm}p{3.2cm}@{}}
\toprule
\textbf{Label} & \textbf{Definition} & \textbf{Example} \\
\midrule
Certain
  & Answers with confidence; no hedging
  & \textit{``It started three days ago.''} \\[3pt]
Approximate\,/\,uncertain
  & Hedges or estimates but still gives an answer
  & \textit{``Maybe three or four days ago.''} \\[3pt]
Doesn't know
  & Explicitly states inability to recall
  & \textit{``I'm not sure, I can't remember.''} \\[3pt]
Contradictory
  & Answer conflicts with something stated earlier
  & Earlier: \textit{``two days ago''} / Later: \textit{``I've had
    this for a month''} \\[3pt]
Refuses to answer
  & Declines to answer
  & \textit{``Just give me the medicine.''} \\[3pt]
N/A & Not a factual history-answer turn & --- \\
\bottomrule
\end{tabular}
\end{table}

\subsection{Physical Examination Layer (Conditional)}
\label{app:metrics:pe}

This layer is activated only for consultations in which the phase
segmentation identifies at least one PE-phase turn. All metrics are
computed over PE-phase turns only.

\medskip
\noindent\textbf{Narration Density (Doctor).}
The proportion of doctor PE turns in which the doctor explicitly
verbalises what they are doing or are about to do during the
examination. E.g., \textit{``I'm going to press your abdomen now''} or
\textit{``Let me listen to your chest.''} Contrasted with turns that
move directly to examination instructions or findings without narrating
the action. Synthetic consultations show substantially higher narration
density than real or simulated comparators, reflecting the tendency of
LLM-generated dialogue to make implicit clinical action verbally
explicit.

\medskip
\noindent\textbf{Deictic Reference Count (Doctor and Patient).}
The number of turns per conversation containing context-bound spatial
or pointing language: \textit{here, there, this side, that area, like
this}, and script-native equivalents. Reported as a rate per PE turn.
High deictic density in real Indian consultations reflects the
context-bound, action-embedded character of physical examination;
its suppression in synthetic data indicates replacement by narrated
or explicitly labelled anatomical references, consistent with LLMs
optimizing for written-text fluency over spoken
interaction~\cite{mayorllmconversations2025}.

\medskip
\noindent\textbf{Findings Disclosure (Doctor).}
The proportion of doctor PE turns in which the doctor explicitly
verbalises examination findings to the patient. E.g., \textit{``Breath
sounds are reduced on the right.''} Contrasted with turns in which
findings are implicit or deferred to the DX phase. Synthetic
consultations disclose findings at higher rates than real or simulated
consultations, mirroring the over-narration pattern in Narration
Density.

\medskip
\noindent\textbf{Compliance--Proactivity (Patient).}
Annotated per patient PE turn. Captures whether patients volunteer
examination-relevant information beyond the doctor's immediate prompt,
distinguishing the reactive compliance characteristic of real Indian
examination interaction from the proactive patient contributions
introduced as a synthetic artefact.

\begin{table}[h]
\small
\caption{Compliance--Proactivity labels (patient PE turns).}
\label{tab:compliance}
\begin{tabular}{@{}p{2.8cm}p{5.0cm}p{3.4cm}@{}}
\toprule
\textbf{Label} & \textbf{Definition} & \textbf{Example} \\
\midrule
Compliant
  & Patient follows the instruction given and nothing more
  & D: \textit{``Deep breath.''} / P: \textit{``Okay.''} \\[4pt]
Proactive
  & Patient volunteers additional examination-relevant information
    or observations beyond what the instruction requested
  & \textit{``Yes --- and actually it also hurts a bit to the right,
    not just there.''} \\
\bottomrule
\end{tabular}
\end{table}

\noindent The \emph{Compliance-Proactivity} metric is the proportion
of patient PE turns labelled Proactive.


==> tables/datasets.tex <==
\begin{table}[t]
\centering
\caption{Datasets used in the evaluation. \textit{Real} = recorded
consultations; \textit{Simulated} = role-played or annotator-written;
\textit{Synthetic} = LLM-generated. en = English, hi = Hindi, te = Telugu.
\textit{Notation} denotes the shorthand to refer to each dataset
throughout the study.}
\label{tab:datasets}
\small
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{@{} p{0.12\linewidth}
                    p{0.12\linewidth}
                    p{0.08\linewidth}
                    p{0.08\linewidth}
                    p{0.50\linewidth} @{}}
\toprule
\textbf{Dataset} & \textbf{Notation} & \textbf{Lang.} & \textbf{Type} & \textbf{Description} \\
\midrule


MTS-Dialog~\cite{ben-abacha-etal-2023-empirical}
  & Sim-US-1
  & en & Simulated
  & \sim$1.7k$ doctor-patient dialogues manually written by healthcare professionals from de-identified real clinical notes \\

ACI-Bench~\cite{yim2023acibench}
  & Sim-US-2
  & en & Simulated
  & 207 doctor-patient encounters constructed by domain experts through role-play each paired with a reference clinical note \\

NoteChat~\cite{wang-etal-2024-notechat}
  & Syn-US-1
  & en & Synthetic
  & GPT-3.5 multi-agent pipeline grounded in PMC case reports \\

Clinical Note Generation ~\cite{ekacare2025clinicalnote}
  & Sim-Indian
  & hi & Simulated
  & 156 transcribed consultations between EkaCare's clinicians and internal staff who role-played as patients, each annotated with structured ground-truth notes. \\

Privtel
  & Real-Indian
  & te & Real
  & Proprietary corpus of real outpatient consultations \\

\midrule
\multicolumn{5}{@{}l}{{Synthetic Generation Setting,
40 samples per cell per language}} \\
\midrule

Free-form, ungrounded
  & Syn-US-2, Syn-Indian-1, Syn-Indian-2
  & en, hi, te & Synthetic
  & Single prompt; model generates an outpatient conversation \\

Free-form, MTS-grounded
  & Syn-US-2, Syn-Indian-1, Syn-Indian-2
  & en, hi, te & Synthetic
  & Single prompt; model seeded with an MTSamples clinical note \\

Agentic, ungrounded
  & Syn-US-2, Syn-Indian-1, Syn-Indian-2
  & en, hi, te & Synthetic
  & Doctor- and patient-agent; no case grounding; $\geq$20 turns \\

Agentic, MTS-grounded
  & Syn-US-2, Syn-Indian-1, Syn-Indian-2
  & en, hi, te & Synthetic
  & Doctor- and patient-agent; MTSamples note as shared grounding;
    $\geq$20 turns \\

\bottomrule
\end{tabular}
\end{table}

==> tables/markers_expanded.tex <==
% requires \usepackage{multirow}
\begin{table*}[t]
\centering
\caption{Cultural-marker annotation framework. \textbf{Spk}: P~=~patient, D~=~doctor, B~=~both.
\textsuperscript{\dag}Exam layer activates only when a physical examination is detected.}
\label{tab:detailed_framework}
\scriptsize
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{@{} p{0.15\linewidth} p{0.17\linewidth} p{0.53\linewidth} c @{}}
\toprule
\textbf{Level (unit)} & \textbf{Metric} & \textbf{Categories / example} & \textbf{Spk} \\
\midrule
\multirow{5}{*}{\shortstack[l]{L0\\Surface\\(dialogue)}}
 & Word counts & Total / mean words per speaker & B \\
 & Turn-length uniformity & Variance in turn length across the conversation & B \\
 & Speaker-alternation regularity & Strict alternation vs.\ runs by one speaker & B \\
 & Backchannel rate & Frequency of tokens like ``mm-hmm,'' ``okay'' & B \\
 & Vocative frequency & Frequency of direct address, e.g.\ ``doctor'' & B \\
\midrule
\multirow{4}{*}{\shortstack[l]{L1\\Phase\\structure\\(turn span)}}
 & Phase label & GR / SE / CC / HT / PE / DX / TX / CL (e.g.\ T01 = greeting) & B \\
 & Phase ordering & Whether phases follow the canonical clinical sequence & B \\
 & Phase duration & Turns per phase & B \\
 & Transition count & Number of phase-to-phase shifts & B \\
\midrule
\multirow{9}{*}{\shortstack[l]{L2\\Turn-level\\(single turn)}}
 & Tone & Directive / Discussive / Empathetic & D \\
 & Verbosity & Terse / Appropriate / Overly verbose & D \\
 & Question structure & Single / Multiple-related / Multiple-unrelated / N/A & D \\
 & Register (multi-select) & Formal clinical / Colloquial / Regional-vernacular / Shorthand & D \\
 & Response style & Structured / Trailing / Deflecting & P \\
 & Info volunteering & Exact / Add-on & P \\
 & Symptom description & Gesture-deictic / Clinical / Colloquial & P \\
 & Response to recommendation (multi-select) & Accepts / Clarifies / Questions / Concern / Refuses / Disagrees / Misunderstands / Alt.-info / Unclear & P \\
 & Certainty & Certain / Approximate / Doesn't know / Contradictory / Refuses & P \\
\midrule
\multirow{4}{*}{\shortstack[l]{Exam\textsuperscript{\dag}\\(exam span)}}
 & Narration density & How much of the exam is verbalized aloud & D \\
 & Deictic reference count & Spatial/pointing language, e.g.\ ``here'' & D \\
 & Findings disclosure & Whether/how findings are shared in real time & D \\
 & Patient compliance & Cooperation with exam instructions & P \\
\midrule
\multirow{5}{*}{\shortstack[l]{L3\\Inter-turn\\(adjacent turns)}}
 & Interruption count/type & Frequency and type of overlapping speech & B \\
 & Doctor echo & Doctor repeats/paraphrases the patient's own words & D \\
 & Topic continuity & Adjacent turns stay on-topic vs.\ shift abruptly & B \\
 & Code-switching & Language/register shift across adjacent turns & B \\
 & Q--A uptake & Whether the patient's answer is taken up next turn & B \\
\bottomrule
\end{tabular}
\end{table*}
